Visualizing the loss landscape of Self-supervised Vision Transformer

The Masked autoencoder (MAE) has drawn attention as a representative self-supervised approach for masked image modeling with vision transformers. However, even though MAE shows better generalization capability than fully supervised training from scratch, the reason why has not been explored. In another line of work, the Reconstruction Consistent Masked Auto Encoder (RC-MAE), has been proposed which adopts a self-distillation scheme in the form of an exponential moving average (EMA) teacher into MAE, and it has been shown that the EMA-teacher performs a conditional gradient correction during optimization. To further investigate the reason for better generalization of the self-supervised ViT when trained by MAE (MAE-ViT) and the effect of the gradient correction of RC-MAE from the perspective of optimization, we visualize the loss landscapes of the self-supervised vision transformer by both MAE and RC-MAE and compare them with the supervised ViT (Sup-ViT). Unlike previous loss landscape visualizations of neural networks based on classification task loss, we visualize the loss landscape of ViT by computing pre-training task loss. Through the lens of loss landscapes, we find two interesting observations: (1) MAE-ViT has a smoother and wider overall loss curvature than Sup-ViT. (2) The EMA-teacher allows MAE to widen the region of convexity in both pretraining and linear probing, leading to quicker convergence. To the best of our knowledge, this work is the first to investigate the self-supervised ViT through the lens of the loss landscape.

==> ack.tex <==
\section{Acknowledgement}
This work was partly supported by Institute of Information \& Communications Technology Planning \& Evaluation(IITP) grant funded by the Korea government(MSIT) (No. RS-2022-00187238, Development of Large Korean Language Model Technology for Efficient Pre-training~(80\%) and No. 2020-0-00004, Development of Previsional Intelligence based on Long-term Visual Memory Network(20\%).

==> fig/epoch.tex <==
\begin{figure*}[t!]
\begin{center}
\scalebox{1.0}{
\includegraphics[width=1.\textwidth]{fig/epoch.pdf}
}
\end{center}
\caption{
% 
\textbf{Loss landscapes of self-supervised vision transformer by MAE~\cite{he2022mae} and RC-MAE~\cite{lee2023rcmae} at different training epochs}. 
Note that as the learning progresses, the optimal point gets sharper.
}
% \vspace{-0.5cm}
\label{fig:epoch}
\end{figure*}

==> fig/epoch_mae.tex <==
\begin{figure*}
\begin{center}
\scalebox{1.0}{
\includegraphics[width=1.\textwidth]{fig/epoch_mae.pdf}
}
\end{center}
\caption{
% 
\textbf{Loss landscapes of self-supervised vision transformer by MAE~\cite{he2022mae} at different pre-training epochs}. 
Note that as the learning progresses, the region close to the optimal point gets sharper.
}
% \vspace{-0.5cm}
\label{fig:mae_epoch}
\end{figure*}

==> fig/mae_pt.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/mae_vit_base_pt_1600ep.pdf}
\end{center}
\vspace{-0.5cm}
\caption{\textbf{Loss landscape visualization} of self-supervised Vision Transformer~\cite{dosovitskiy2021vit} by Masked Autoencoder~(MAE~\cite{he2022mae}). 
Note that this loss landscape is computed as a pre-training loss~(\eg, masked patch reconstruction task), not a classification task.}
\label{fig:mae_pt}
\vspace{-0.2cm}
\end{figure}

==> fig/mae_vs_rc.tex <==
\begin{figure}[h]
\begin{center}
\scalebox{1.0}{
\includegraphics[width=0.98\linewidth]{fig/mae_vs_rc.pdf}
}
\end{center}
\caption{
% 
\textbf{Architectures of MAE~\cite{he2022mae} and RC-MAE~\cite{lee2023rcmae}.}
RC-MAE adds a teacher network to MAE, considering MAE as a student network.
In RC-MAE, the student network~(MAE) is optimized by a reconstruction loss~(\textbf{\textcolor{cobalt}{$\loss{r}$}}) with input image target and a consistency loss~(\textbf{\textcolor{Mahogany}{$\loss{c}$}}) with the teachers' reconstructed target.
}
% \vspace{-0.3cm}
\label{fig:arch}
\end{figure}
